Taming Reachability Analysis of DNN-Controlled Systems via Abstraction-Based Training

The intrinsic complexity of deep neural networks (DNNs) makes it challenging to verify not only the networks themselves but also the hosting DNN-controlled systems. Reachability analysis of these systems faces the same challenge. Existing approaches rely on over-approximating DNNs using simpler polynomial models. However, they suffer from low efficiency and large overestimation, and are restricted to specific types of DNNs. This paper presents a novel abstraction-based approach to bypass the crux of over-approximating DNNs in reachability analysis. Specifically, we extend conventional DNNs by inserting an additional abstraction layer, which abstracts a real number to an interval for training. The inserted abstraction layer ensures that the values represented by an interval are indistinguishable to the network for both training and decision-making. Leveraging this, we devise the first black-box reachability analysis approach for DNN-controlled systems, where trained DNNs are only queried as black-box oracles for the actions on abstract states. Our approach is sound, tight, efficient, and agnostic to any DNN type and size. The experimental results on a wide range of benchmarks show that the DNNs trained by using our approach exhibit comparable performance, while the reachability analysis of the corresponding systems becomes more amenable with significant tightness and efficiency improvement over the state-of-the-art white-box approaches.

==> validity.tex <==
%\vspace{-1mm}
%\subsection{Threats to Validity}
%\vspace{-1mm}
% are very complex and usually operate under uncertain environments. 
\zm{arg1}{Delete this section or move to Conclusion sec.?} There are two main threats to the validity of the proposed approach due to the intrinsic complexity of DNN-controlled systems and their uncertain running environments.
\vskip 1ex 
\noindent\textbf{High-dimensional systems.} Dimensionality is always  one of the central threats to reachability analysis. All the relevant approaches are  facing the curse of dimensionality~\cite{ivanov2021verisig,huang2019reachnn,huang2022polar}. 
Thanks to the representation power of DNNs \cite{tuckerman2022curse}, our training approach can support training DNNs for high-dimensional systems because the complexity of transforming an $n$-dimensional state into an interval box is $O(n)$. Nevertheless, the reachability analysis part may suffer from state explosion in the worst case when the number of reachable states increases  exponentially as the system proceeds. One possible solution to this threat is to coarsen the abstraction to reduce the size of abstract states, and learn an easy-to-verify linear policy for those states mapped to the same coarsened abstract state. Such an approach has been successfully applied to reinforcement learning \cite{akrour2018regularizing} and requires further investigation into the DNN-based cases. 

%The curse of  dimensionality always exist and 

\vskip 1ex 
\noindent\textbf{Complex environment dynamics.} 
Environment dynamics is another threat, as faced by all the formal verification approaches to hybrid systems. An environment dynamics in the real world can be as complex as chaotic~\cite{immler2015verified}, which may produce divergent traces and lead to an uncontrollable explosion of overestimation even to those systems controlled by programmatic controllers. It is out of the scope of this work to investigate tight over-approximation for complex environment dynamics. 
%For the embedded neural network controller, small-sized neural networks may not be able to fit the optimal state-action policy due to its limited expressivity when facing complex dynamics.




\color{black}
